The Heavy Hitter Oracle: Enhancing Frequency Estimation in Skewed Data Streams

Estimating element frequencies in data streams is a fundamental problem when processing large amounts of data. Recent approaches suggest learning-augmented algorithms that can access a heavy-hitter oracle that knows the most frequent elements. In this paper, we challenge the idea of these complex oracles: First, we show that heavy-hitter predictions do not necessarily yield significant efficiency gains in frequency estimation. We prove that a classical algorithm using slightly more memory, $\Theta(B \log B)$ instead of $\Theta(B)$, matches the performance of learning-augmented methods with perfect predictions. Furthermore, we show that given (perfect) predictions, a trivial mechanism achieves the same performance as state-of-the-art learning-augmented algorithms. On the algorithmic side, we introduce $\textit{SpaceR}$, a single-pass algorithm that matches the accuracy of existing two-pass prediction-based methods without requiring any predictions. SpaceR uses randomized sampling to identify and track frequent elements in one pass through the data, achieving near-perfect frequency recovery with minimal memory on both synthetic and real-world datasets.

==> Chapters/07_Acknowledgements.tex <==
\section*{Acknowledgement}

==> Chapters/08_Impact_Statement.tex <==
\section*{Impact Statement}
This paper presents work whose goal is to advance the field of Machine
Learning. There are many potential societal consequences of our work, none
which we feel must be specifically highlighted here.

==> preamble.tex <==
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
%                           PACKAGES                                 %
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
\usepackage[separate-uncertainty=true,reset-math-version=false,detect-weight=true,detect-family=true]{siunitx}
\usepackage{silence}
\WarningFilter*{hyperref}{Token not allowed in a PDF string}
\WarningsOff[caption]
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{tabularx}
\usepackage{lipsum}
\usepackage{url}
\usepackage{placeins}
\usepackage{booktabs}
\usepackage{soul}
\usepackage{amsfonts}
\usepackage{nicefrac}
\usepackage{microtype}
%\usepackage[numbers]{natbib}
%\usepackage{proba}
\usepackage{wrapfig}
\usepackage{caption}
\usepackage{amssymb}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\usepackage{subcaption}
\usepackage{float}
\usepackage{rotating}
\usepackage{etoolbox}
\usepackage{xparse}
\usepackage{grffile}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{euscript}
\usepackage{enumitem}
\usepackage{mathtools}
\usepackage{tikz}
\usepackage{tablefootnote}
\usepackage[flushleft]{threeparttable}
\usepackage{multirow}
\usepackage[title]{appendix}
\usepackage{arydshln}
\usepackage{array, booktabs}
\usepackage{comment}
\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage{amsmath,amsthm}
\usepackage{dsfont}
\usepackage{balance}
\usepackage{multicol}
\usepackage{xcolor}
\usepackage{nameref}
\usepackage{pdfpages}
\usepackage{braket}
\usepackage[normalem]{ulem}
\usepackage{bbding}
% \usepackage[capitalise, noabbrev, nameinlink]{cleveref}
\usepackage{xfrac}
\usepackage[usestackEOL]{stackengine}
\usepackage{indentfirst}
\usepackage{csquotes}
\usepackage{pgf}
\usepackage{varwidth}
\usepackage{verbatimbox}
\usepackage{verbatim}
\usepackage{bm}
\usepackage{anyfontsize}
\usepackage{todonotes}
\usepackage[svgnames]{xcolor}

\usepackage{empheq}
\definecolor{myblue}{rgb}{.8, .8, 1}
\newcommand*\mybluebox[1]{%
\colorbox{myblue}{\hspace{1em}#1\hspace{1em}}}

% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
%                           CAPTION SETTINGS                         %
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%

\captionsetup{font=small}
\captionsetup[sub]{font=small}
\captionsetup[subfigure]{labelformat = parens, labelsep = space, font = small}
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
%                         COLOR MACROS                               %
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%

\definecolor{pastelblue}{RGB}{76,113,175}
\definecolor{pastelgreen}{RGB}{144,238,144}
\definecolor{pastelred}{RGB}{196,78,82}
\definecolor{pastelgrey}{RGB}{230,230,230}
\definecolor{pastelbeige}{RGB}{243,236,221}
\definecolor{pastelpurple}{RGB}{154,139,192}
\definecolor{salmon}{RGB}{250, 128, 114}
\definecolor{darkgreen}{rgb}{0,0.6,0}
\definecolor{darkred}{rgb}{0.5,0,0}
\definecolor{verylightgreen}{HTML}{F6FFF9}
\definecolor{verylightred}{HTML}{FFF4F3}
\definecolor{verylightgray}{HTML}{F4F6F6}
\definecolor{babyblueeyes}{rgb}{0.63, 0.79, 0.95}
\definecolor{lightpink}{rgb}{1.00, 0.714, 0.757}


% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
%                         THEOREM ENVIRONMENTS                       %
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%

% \newtheorem{theorem}{Theorem}
% \newtheorem*{theorem*}{Theorem}
% \newtheorem{assumption}{Assumption}
% \newtheorem{axiom}{Axiom}
% \newtheorem{case}{Case}
% \newtheorem{claim}{Claim}
% \newtheorem{conclusion}{Conclusion}
% \newtheorem{condition}{Condition}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{corollary}{Corollary}
% \newtheorem{criterion}{Criterion}
% \newtheorem{definition}{Definition}
% \newtheorem{exercise}{Exercise}
% \newtheorem{example}{Example}
% \newtheorem{lemma}{Lemma}
% \newtheorem{notation}{Notation}
% \newtheorem{problem}{Problem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{property}{Property}
% \newtheorem{solution}{Solution}
% \newtheorem{summary}{Summary}
% \newtheorem{motivation}{Motivation}
% \newtheorem{query}{Query}
% \newtheorem{observation}{Observation}
% %\theoremstyle{remark}
% \newtheorem{remark}{Remark}

% Let cleveref and thmtools work together
\makeatletter
\def\thmt@refnamewithcomma #1#2#3,#4,#5\@nil{%
	\@xa\def\csname\thmt@envname #1utorefname\endcsname{#3}%
	\ifcsname #2refname\endcsname
	\csname #2refname\expandafter\endcsname\expandafter{\thmt@envname}{#3}{#4}%
	\fi}
\makeatother
\crefname{equation}{Equation}{Equations}
\crefname{section}{Section}{Sections}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{proposition}{Proposition}{Propositions}
\crefname{appendix}{Appendix}{Appendices}
\crefname{theorem}{Theorem}{Theorems}
\crefname{figure}{Figure}{Figures}
\crefname{tabular}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithm}
\Crefname{conjecture}{Conjecture}{Conjectures}
\Crefname{definition}{Definition}{Definitions}
\Crefname{observation}{Observation}{Observations}
\Crefname{assumption}{Assumption}{Assumptions}
\Crefname{axiom}{Axiom}{Axioms}
\Crefname{case}{Case}{Cases}
\Crefname{claim}{Claim}{Claims}
\Crefname{conclusion}{Conclusion}{Conclusions}
\Crefname{condition}{Condition}{Conditions}
\Crefname{criterion}{Criterion}{Criteria}
\Crefname{exercise}{Exercise}{Exercises}
\Crefname{example}{Example}{Examples}
\Crefname{notation}{Notation}{Notations}
\Crefname{problem}{Problem}{Problems}
\Crefname{property}{Property}{Properties}
\Crefname{remark}{Remark}{Remarks}
\Crefname{solution}{Solution}{Solutions}
\Crefname{summary}{Summary}{Summaries}
\Crefname{motivation}{Motivation}{Motivations}
\Crefname{query}{Query}{Queries}
\newcommand{\algorithmautorefname}{Algorithm}
\newcommand*{\Appendixautorefname}{Appendix}
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
%                           MATH MACROS                              %
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
\newcommand{\mathcolorbox}[2]{\colorbox{#1}{$\displaystyle #2$}}
\newcommand{\one}{\mathds{1}}
\newcommand{\negquad}{\mkern-18mu}
\newcommand{\red}[1]{{\color{red} #1}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand*\dbar[1]{\overline{\overline{\lower0.2ex\hbox{$#1$}}}}
\newcommand{\supp}{\text{supp\xspace}}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\dom}{\text{dom}}
\newcommand{\ran}{\text{ran}}
\newcommand{\setsize}[1]{\mid \! #1 \! \mid}
\def\th{^{\text{th}}}
%Stats macros:
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\pr}{P}
\newcommand{\Exp}{\mathds{E}}
\newcommand{\eqdist}{\stackrel{d}{=}}
\newcommand{\eqas}{\stackrel{\text{a.s.}}{=}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\indep}{\perp\!\!\!\perp}
%Causality macros
\newcommand{\doop}{\text{do}}
\newcommand{\Parents}{\text{Pa}}
\newcommand{\parents}{\text{pa}}
%Graph macros
\newcommand{\iso}{\cong}
\newcommand{\notiso}{\not cong}
\newcommand{\aut}[1]{\text{Aut}(#1)}
%Machine learning macros:
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\lf}{\mathcal{L}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\relu}{\text{ReLU}}
%Font macros
\def\cA{{\mathcal{A}}}
\def\cB{{\mathcal{B}}}
\def\cC{{\mathcal{C}}}
\def\cD{{\mathcal{D}}}
\def\cE{{\mathcal{E}}}
\def\cF{{\mathcal{F}}}
\def\cG{{\mathcal{G}}}
\def\cH{{\mathcal{H}}}
\def\cI{{\mathcal{I}}}
\def\cJ{{\mathcal{J}}}
\def\cK{{\mathcal{K}}}
\def\cL{{\mathcal{L}}}
\def\cM{{\mathcal{M}}}
\def\cN{{\mathcal{N}}}
\def\cO{{\mathcal{O}}}
\def\cP{{\mathcal{P}}}
\def\cQ{{\mathcal{Q}}}
\def\cR{{\mathcal{R}}}
\def\cS{{\mathcal{S}}}
\def\cT{{\mathcal{T}}}
\def\cU{{\mathcal{U}}}
\def\cV{{\mathcal{V}}}
\def\cW{{\mathcal{W}}}
\def\cX{{\mathcal{X}}}
\def\cY{{\mathcal{Y}}}
\def\cZ{{\mathcal{Z}}}
\def\bA{{\bm{A}}}
\def\bB{{\bm{B}}}
\def\bC{{\bm{C}}}
\def\bD{{\bm{D}}}
\def\bE{{\bm{E}}}
\def\bF{{\bm{F}}}
\def\bG{{\bm{G}}}
\def\bH{{\bm{H}}}
\def\bI{{\bm{I}}}
\def\bJ{{\bm{J}}}
\def\bK{{\bm{K}}}
\def\bL{{\bm{L}}}
\def\bM{{\bm{M}}}
\def\bN{{\bm{N}}}
\def\bO{{\bm{O}}}
\def\bP{{\bm{P}}}
\def\bQ{{\bm{Q}}}
\def\bR{{\bm{R}}}
\def\bS{{\bm{S}}}
\def\bT{{\bm{T}}}
\def\bU{{\bm{U}}}
\def\bV{{\bm{V}}}
\def\bW{{\bm{W}}}
\def\bX{{\bm{X}}}
\def\bY{{\bm{Y}}}
\def\bZ{{\bm{Z}}}
\def\ba{{\bm{a}}}
\def\bb{{\bm{b}}}
\def\bc{{\bm{c}}}
\def\bd{{\bm{d}}}
\def\be{{\bm{e}}}
%\def\bf{{\bm{f}}}
\def\bg{{\bm{g}}}
\def\bh{{\bm{h}}}
\def\bi{{\bm{i}}}
\def\bj{{\bm{j}}}
\def\bk{{\bm{k}}}
\def\bl{{\bm{l}}}
\def\bbm{{\bm{m}}}
\def\bn{{\bm{n}}}
\def\bo{{\bm{o}}}
\def\bp{{\bm{p}}}
\def\bq{{\bm{q}}}
\def\br{{\bm{r}}}
\def\bs{{\bm{s}}}
\def\bt{{\bm{t}}}
\def\bu{{\bm{u}}}
\def\bv{{\bm{v}}}
\def\bw{{\bm{w}}}
\def\bx{{\bm{x}}}
\def\by{{\bm{y}}}
\def\bz{{\bm{z}}}
%For multiset notation
\newcommand*{\lms}{\{\mskip-5mu\{}
\newcommand*{\rms}{\}\mskip-5mu\}}

% For probabilities
\newcommand{\cond}{\,|\,}

\newcommand{\crefrangeconjunction}{--}

% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%
%                         MATH FONT COMMANDS                         %
% -===============                                    ===============%
% -===============                                    ===============%
% -===============                                    ===============%

\DeclareFontFamily{U}{BOONDOX-calo}{\skewchar\font=45 }
\DeclareFontShape{U}{BOONDOX-calo}{m}{n}{
  <-> s*[1.05] BOONDOX-r-calo}{}
\DeclareFontShape{U}{BOONDOX-calo}{b}{n}{
  <-> s*[1.05] BOONDOX-b-calo}{}
\DeclareMathAlphabet{\mathcalb}{U}{BOONDOX-calo}{m}{n}
\SetMathAlphabet{\mathcalb}{bold}{U}{BOONDOX-calo}{b}{n}
\DeclareMathAlphabet{\mathbcalb}{U}{BOONDOX-calo}{b}{n}
\newcommand{\sff}[1]{ \text{ {\sffamily \textbf{  {#1} }} } }
\newcommand{\ecal}[1]{ \EuScript{#1} }

%% Removes commands not allowed in PDF fields, such as line breaks
\pdfstringdefDisableCommands{%
  \def\\{}%
  \def\texttt#1{<#1>}%
}

% Convenience for linewidth specifically

\usepackage{xfp}
\ExplSyntaxOn
% \printdimall[<decimals>]{<dimension>}
\newcommand{\printdimall}[2][4]{%
  \begingroup\leavevmode
  \fpeval{ round( \dim_to_fp:n {#2} , #1 ) }\,pt%
  \space(%
    \fpeval{ round( \dim_to_fp:n {#2} / \dim_to_fp:n {1cm} , #1 ) }\,cm; %
    \fpeval{ round( \dim_to_fp:n {#2} / \dim_to_fp:n {1in} , #1 ) }\,in%
  )%
  \endgroup
}

% Convenience for \linewidth
\newcommand{\printlinewidth}[1][4]{\printdimall[#1]{\linewidth}}
\ExplSyntaxOff

\newcommand\thefontsize{The current font size is: \f@size pt}
